Orthogonal Time Frequency Space (OTFS) Modulation for Wireless Communications

Orthogonal time frequency space (OTFS) modulation is a recently proposed multi-carrier transmission scheme, which innovatively multiplexes the information symbols in the delay-Doppler (DD) domain instead of the conventional time-frequency (TF) domain. The DD domain symbol multiplexing gives rise to a direct interaction between the DD domain information symbols and DD domain channel responses, which are usually quasi-static, compact, separable, and potentially sparse. Therefore, OTFS modulation enjoys appealing advantages over the conventional orthogonal frequency-division multiplexing (OFDM) modulation for wireless communications. In this thesis, we investigate the related subjects of OTFS modulation for wireless communications, specifically focusing on its signal detection, performance analysis, and applications. These important aspects are discussed based on the review of the state-of-the-art and a detailed derivation of OTFS modulation from the discrete Zak transform (DZT). Finally, a summary of future research directions on OTFS modulation are also provided.

==> 1-pre/ack.tex <==
\chapter{Acknowledgement}
I would like to express the most sincere gratitude to my Ph. D. supervisor Prof. Jinhong Yuan, who has been very supportive to my research and my career. He is a more like a mentor to me, who has not only taught me how to conduct research but also educated me what is the right attitude towards life. I could not accomplish this thesis without his support and education. I really appreciate his rigorous and optimistic attitude towards research, which have inspired me so much. There are two things I remember the most. One is that he taught me to look for the big problem (in his words could be ``do not throw away the watermelon for the sesame''). Another one is to look for the physical meanings behind the math. Those words and advices from him have always been the
guidelines for me every time I work on a research problem.
I would also like to thank him for his strong supports in my research, which paves the way for my future career. He has offered me endless opportunities including collaborations with both industry and academic, which I consider meaningful and unforgettable. In summary, he truly is an educator. He educated me how to be a real researcher.

I would like to thank my co-supervisors, Dr. Lei Yang, and Prof. Derrick Wing Kwan Ng, for their valuable inputs that contribute to my research. I owe my thanks to Dr. Lei Yang for his help and efforts in discussing with me for the related research. I am also very grateful to Prof. Derrick Wing Kwan Ng, who has spent countless times helping me with the research and my career. Derrick is a mentor and a friend, who always shares his professional views on the research to all his students. Derrick's encouragement and experience are very helpful to me to overcome the most difficult time, especially in my early stage of my Ph.D. study. I learned quite a lot from him and I will always cherish him as a big brother and a role model as a good researcher.

I owe my gratitude to my previous supervisor Prof. Baoming Bai in Xidian University, who has introduced me to the research of communication. I really appreciate the efforts he made to help me with my understanding of the basic knowledge of the field. On top of that, he always shares his views and gives insightful instructions to his students. I sincerely thank him for giving me the opportunity to study abroad and introducing me to Prof. Yuan. I would not achieve this much without his help and encouragements, for which I will be always grateful.

I would like to thank all the teachers I met during my Ph. D. journey. I want to thank Prof. Giuseppe Caire, Prof. Shu Lin, Prof. Lajos Hanzo, Prof. Xiao Ma, Prof. Nevio Benvenuto, Prof. Qinghua Guo, Prof. Yonghui Li, Dr. Yixuan Xie, Prof. Yu-Chih (Jerry) Huang, Prof. Tongxing Zheng, Prof. Fan Liu, and Dr. Yuanhao Cui. I highly value the helpful instructions they have offered me and I really have learned a lot from all of them.

I am very fortunate to be part of a member of the wireless communication group of the University of New South Wales. All those happy moments and valuable encouragements during my study will always be a wonderful experience in my life. I would thank Prof. Lou Zhao, Prof. Zhuo Sun, Dr. Min Qiu, Dr. Zhiqiang Wei, Dr. Weijie Yuan, Dr. Chang Liu, Prof. Shihao Yan, Dr. Qingqing Cheng, Dr. Sachini Jayasooriya, Dr. Peng Kang, Dr. Bryan Liu, Dr. Xiaowei Wu, Dr. Yuanxin Cai, Mr. Yihuan Liao, Mrs. Shaokang Hu, Mr. Hamish Shaw, Mr. Qi (Oliver) Li, Mr. Cheng Shen, and Mr. Chong Zhang. Specially, I want to thank Prof. Weijie Yuan, and Dr. Zhiqiang Wei for always having research discussions with me. This thesis could not be accomplished without your help.

I want to thank the members in the ISN lab in Xidian university. Thank you Prof. Bing Li, Prof. Min Zhu, Prof. Hengzhou Xu, Ms. Rui Zhang, Dr. Xijin Mu, Dr. Dan Feng, Dr. Peiyao Chen, Dr. Huaan Li, Dr. Zhongyang Yu, Mrs. Qingya Lu, Mr. Hefang Guan, Mr. Fei Wan, Ms. Mengmeng Liu, Mr. Rongchi Xu, Mr. Cheng Sun, Mr. Gang Chen, Ms. Chunhui Shen, Mr. Lei Ping, Mr. Hao Sun, Ms. Chen Qiu, Mr. Xiaonan Ruan, Mrs. Qiang Zhang, Ms. Minzi Xu, Ms. Qian Li, Mr. Dixia Deng, Ms. Qingli He, Mr. Zhaofeng Ren, Ms. Xue Tan, Mr. Fuwei Huang, Ms. Mengmeng Liu, Ms. Xin Dou, Mr. Jipeng Zhang, Mr. Zhen Liu, Ms. Xiaoying Wang, Ms. Zhixin Hu, Mr. Lei Wu, Mr. Dianhao Hou, Mr. Binghao Li, Mr. Shenyang Zhou, Ms. Jiayi Zhang, Ms. Chunqiong Zhang, Ms. Ruixue Gao, Mr. Zhenyu Shen, Mr. Yuan Wang, Mr. Ruimin Yuan, Ms. Chenxi Si. Specially, I want to thank Prof. Bing Li, Dr. Peiyao Chen, Dr. Dan Feng, Dr. Xijin Mu, Dr. Zhongyang Yu, Ms. Mengmeng Liu, Ms. Qian Li, and Ms. Chenxi Si for their help for my research.


I want to thank my girlfriend Ruoxi Chong for her kind support and tolerance. She offered endless help to me during the difficult times, for which I will never forget. I am very grateful to her for all the help and encouragement to me.

In the end, I would like to use this opportunity to thank my parents for their kindness and support for me during the last 30 years. Their nurturing love is irreplaceable. I would also like to thank all my friends for accompanying me through this Ph. D. journey. Thank you all very much.


==> 3-literature/literature_review.tex <==
\chapter{Literature Review}\label{c:literature}

The technology of OTFS modulation has been developed rapidly ever since the pioneering paper of Hadani, \emph{et. al.}~\cite{Hadani2017orthogonal}, and several summaries about
the developments of OTFS modulation have also appeared in the literature~\cite{hadani2018whitebook,Zhiqiang_magzine,Shuangyang2021tutorial}.
In this chapter, we aim to provide a literature review of the recent advances of OTFS modulation. In particular, we will summarize the related works of OTFS modulation based on different subjects of the topic, including: OTFS concept and implementation, channel estimation, signal detection, performance analysis, and applications.

\section{OTFS Concept and Implementation}
The concept of OTFS modulation was built upon the elegant mathematical theory of ZT~\cite{zak1967finite,janssen1988zak}, but the intrinsic connections between OTFS modulation and ZT were not discussed in detail in the first paper of OTFS~\cite{Hadani2017orthogonal}. In~\cite{mohammed2021derivation}, the author provided an interesting interpretation of OTFS from the ZT point of view, where a rigorous derivation of OTFS modulation from the first principles is given. In particular, some important and interesting properties of OTFS modulation have been discussed and explained, such as the twisted convolution, DD domain localization. A recent work~\cite{lampel2021orthogonal} also gives a direct implementation of OTFS modulation based on the DZT~\cite{Bolcskei1994Gabor,bolcskei1997discrete}, where the authors have shown that the OTFS modulation can be simply implemented by a DZT transformation. More importantly, this paper also considered the pulse shaping issue of OTFS modulation from the DD domain interpretations, where insightful conclusions are also obtained.

Although the OTFS modulation can be directly implemented in the DD domain via ZT/DZT, the implementation of OTFS modulation via the TF domain has also been widely considered in the literature~\cite{Hadani2017orthogonal,Hadani2018OTFS_long}. The idea of the TF domain implementation is first to transform the DD domain information symbols into the TF domain by using the inverse symplectic finite Fourier transform (ISFFT) and then modulates the TF domain symbols based on conventional TF domain multi-carrier modulators, such as OFDM modulator~\cite{hadani2018whitebook}.
Furthermore, depending on how to insert the cyclic prefix (CP), there are two types OTFS appeared in the literature, namely ZT/DZT-based OTFS~\cite{mohammed2021derivation,lampel2021orthogonal} and CP/OFDM-based OTFS~\cite{rezazadehreyhani2018analysis}. In specific, the ZT/DZT-based OTFS only requires one CP in the time-delay (TD) domain and consequently, there will be interference in both the TF domain and DD domain at the receiver side. Some derivations on the ZT/DZT-based OTFS, including the input-output relationship among different domains, could be found in~\cite{Raviteja2018interference} and~\cite{Raviteja2019practical}{\footnote{Strictly speaking, the work of~\cite{Raviteja2018interference} considered the zero-padding technique instead of inserting CP. However, it has been shown that the resultant input-output relationship is similar to the ZT/DZT-based OTFS~\cite{pandey2021low}. }}.
On the other hand, the CP/OFDM-based OTFS appends the CP similar to the conventional CP insertion for OFDM modulation, e.g., each OFDM symbol contains one CP. Therefore, after the CP removal, the resultant TF domain symbols will have no intersymbol interference (ISI)~\cite{rezazadehreyhani2018analysis}. A concise system model for CP/OFDM-based OTFS has been demonstrated in~\cite{rezazadehreyhani2018analysis}. It can be shown that these two implementations have distinct properties, and we will provide more detailed discussions on DZT-based OTFS in Chapter~3.

The connections between OTFS modulation and conventional multi-carrier modulation schemes have also been discussed in the literature. For example, the connection between OTFS modulation and the generalized frequency-division multiplexing (GFDM) modulation was discussed in~\cite{nimr2018extended}, where the authors have shown that OTFS modulation could be implemented based on GFDM framework with a simple permutation. In particular, the authors have shown that the permutation is the key ingredient for achieving the promising performance over practical wireless channels. The connections between OTFS modulation and other schemes, such as vector OFDM (VOFDM) modulation, and orthogonal short time Fourier (OSTF) modulation, have also been discussed before, and we refer the interested readers to~\cite{Yao2021OTFS} and~\cite{sayeed2021time} for more details.
\section{Channel Estimation}
The channel estimation is an important issue for OTFS systems.
In comparison to the conventional channel estimation in the TF domain, OTFS modulation enables DD domain channel estimation approach that could capture the DD domain channel response with a reduced signaling overhead. Perhaps, the most famous channel estimation scheme is the one proposed in~\cite{Raviteja2019embedded}. In~\cite{Raviteja2019embedded}, an embedded pilot scheme for OTFS channel estimation has been proposed, where a sufficiently large guard interval is applied around the pilot to improve the acquisition of delay and Doppler responses. As the DD domain interaction between the transmitted signal and the channel response can be characterized by the twisted convolution, such a scheme can result in direct channel estimation by simply checking the received signal's value around the DD grid of the embedded pilot.
This approach has soon be extended to the multiple-input multiple-output (MIMO) case in~\cite{Ramachandran2018mimo}, where several pilot symbols are inserted
for different transmit antennas with sufficient guard spacing in the DD domain.
Although~\cite{Raviteja2019embedded} has offered a very simple and direct channel estimation framework, it may require a large guard space to perform well, especially when the DD domain channel sparsity does not hold, e.g., fractional Doppler case.
To overcome this issue, a superimposed pilot scheme has been considered in~\cite{Weijie2021superimposed}, where there is no guard interval around the pilot, such that the signaling overhead is minimized. Consequently, an iterative receiver is adopted to recover the superposition between pilot and information symbols, and the simulation results showed a similar error performance to that of~\cite{Raviteja2019embedded} at an expense of higher computation complexity.
Meanwhile. several compressed sensing-based approaches have been studied in the literature. For instance, the
authors in~\cite{Wenqian2019channel} proposed a three-dimensional (3D) structured orthogonal matching pursuit (SOMP) algorithm to estimate the delay-Doppler-angle domain channel via exploiting the 3D structured sparsity.
A 3D Newtonized orthogonal matching pursuit (NOMP) algorithm was proposed in~\cite{Muye2021new_path}, which exploits the fractional component in the Doppler and angle domains via Newton's method.
Furthermore, some recent works on channel estimation based on sparse Bayesian learning approaches have also appeared in~\cite{Lei2020sparse,Wei2021off,Zhiqiang2021new_offgrid}, which have demonstrated better error performances compared to the orthogonal matching pursuit-based approaches.


\section{Signal Detection}
The signal equalization for OTFS has also been a widely studied subject.
Many existing studies focused on the low-complexity detection for OTFS modulation.
In \cite{Raviteja2018interference}, the authors developed an iterative receiver based on the classic message passing algorithm, where the interference from other information symbols is treated as a Gaussian variable to reduce the detection complexity. However, due to the short cycles on probabilistic graphical model, MPA may fail to converge and results in performance degradation.
To solve this issue, the authors of \cite{Yuan2019simple} proposed a convergence guaranteed receiver based on the variational Bayes framework.
The basic idea of this detector is to approximate the corresponding \emph{a posteriori} distribution of the optimal detection by exploiting the Kullback-Leibler (KL) divergence such that the message passing algorithm can be implemented based on a simpler graphical model. %compared to that of the original OTFS modulation.
A hybrid detection scheme is proposed in~\cite{li2021hybrid}, where both MAP detection and PIC detection are considered according to the channel coefficients. Simulation results show that this hybrid detection can approach the error performance of near-optimal symbol-wise MAP detection, especially for coded OTFS systems, but only requires a reduced complexity.
An OTFS detection approach based on approximate message passing (AMP) with a unitary transformation (UAMP) developed in~\cite{yuan2020iterative}, which not only enjoys a strong resilience to the error propagation due to the short cycles on probabilistic graphical model but also enables an efficient implementation.
Two DD domain low-complexity linear equalizers for OTFS modulations were studied in~\cite{Surabhi2020low}, where the authors proposed simplified implementation of linear minimum mean squared error (L-MMSE) and zero-forcing (ZF) detections with only a logarithmic complexity by exploiting the DD domain channel properties.
A Rake-receiver based OTFS detection was proposed in~\cite{Tharaj2020low_complexity}, where the zero-padding technique was also adopted to shape the corresponding channel matrix to assist the application of DD domain maximum ratio combining.

It should be noticed that most of the existing works on the OTFS detection take advantage of the DD domain channel sparsity to reduce the detection complexity.
However, when an OTFS frame duration is not sufficiently long, the resultant DD domain effective channel can be dense due to the insufficient resolution of the Doppler frequency, i.e., fractional Doppler~\cite{Raviteja2018interference}. In such a case, conventional detection methods may experience a very high detection complexity since the channel sparsity no longer holds.
In light of this, a cross domain iterative detection was proposed in~\cite{li2021cross}, where the extrinsic information is passed between the TD domain and DD domain via the corresponding unitary transformations in order to improve the error performance.
\section{Performance Analysis}
The unique properties of OTFS modulation has gives rise to various advantages for the practical system design. For example, it has been reported that OTFS modulation enjoys the potential of achieving full channel diversity~\cite{Hadani2017orthogonal,Hadani2018OTFS_long}. In specific, the diversity performance of uncoded OTFS signals has been studied in~\cite{Surabhi2019on}, where the authors have shown that the diversity gain of uncoded OTFS systems can be one but the full diversity can be obtained by suitable precoding schemes. The \emph{effective} diversity was discussed in~\cite{Raviteja2019effective}, where the authors have shown that the the full diversity can be achieved almost surely for the case of two resolvable paths when the frame size is sufficiently large, even for uncoded OTFS modulation systems.

The error performance of coded OTFS systems has been investigated in~\cite{li2021performance_analysis,Li2020on}, where the authors have shown that there is a trade-off between the diversity gain and the coding gain of OTFS systems. In particular, it has been shown in~\cite{li2021performance_analysis,Li2020on} that the diversity gain of OTFS systems improves with the number of resolvable paths, while the coding gain declines, which provided some insightful code design guidelines. Furthermore, the correctness of this conclusion has been verified in~\cite{liu2022coded}, where extensive simulation with state-of-art channel coding schemes are demonstrated.
The error performance of OTFS systems with carefully designed TF domain windows has been studied in~\cite{wei2020transmitter}, where the authors have shown that the TF domain windowing could effectively mitigate the Doppler effect from the channel and improve the channel estimation performance.
The achievable rate for CP/OFDM-based OTFS systems was studied in~\cite{rezazadehreyhani2018analysis}. In particular, it is shown that both CP/OFDM-based OTFS and conventional OFDM systems share the same achievable rate, due to the unitary transformation between TF and DD domains.
The pragmatic capacities of both OTFS and OFDM were compared in~\cite{Gaudio2021fair_comparison}, where the achievable rates of both OTFS and OFDM are computed under practical channel estimation and signal detection schemes. In particular, it is shown in~\cite{Gaudio2021fair_comparison} that the pragmatic capacity of OTFS outperforms the OFDM counterpart, especially in the presence of severe Doppler effect.
In~\cite{Surabhi2019peak}, the peak-to-average power ratio (PAPR) of OTFS modulation was investigated, which has shown that OTFS modulation has a better PAPR performance than that of OFDM modulation and GFDM modulation. In particular, the authors have shown that the PAPR of OTFS waveform is proportionate to the number of Doppler bins/time slots instead of number of delay bins/sub-carriers. Therefore, it generally enjoys a relatively low PAPR in practical systems.
\section{Applications}
The success of OTFS has attracted many applications. In this section, we will mainly review some recent works on those applications, such as multiple access transmissions and ISAC.
\subsection{Multiple Access Transmissions}
In light of the advantages of OTFS modulation over the conventional OFDM modulation~\cite{Zhiqiang_magzine}, it is natural to investigate the multiple access schemes based on OTFS modulation to realize robust multi-user transmissions in high-mobility environments. For instance, a path-division multiple access scheme was proposed in~\cite{Muye2021new_path}, where the inter-user interference for downlink transmission is significantly suppressed by a low complexity beamforming design. Also, a study on DD domain multiple access schemes was reported in~\cite{surabhi2019multiple}, where the authors have shown the bit error rate (BER) advantages of the DD domain multiple access schemes over the conventional OFDM counterpart via simulations. The achievable rate upper-bounds for DD domain multiple access schemes have been studied in~\cite{Ruoxi2022achievable}, where the authors derived upper-bounds for both delay division multiple access scheme and Doppler division multiple access scheme. Furthermore, it is shown in~\cite{Ruoxi2022achievable} that the OTFS modulation has an achievable rate upper-bound that is independent from the delay and Doppler distributions, thanks to the ``channel hardening'' effect. However, the achievable rate upper-bound for the OFDM counterpart depends highly on the delay and Doppler distributions, due to the inevitable TF domain superposition among resolvable paths. Consequently, it is shown that DD domain multiple access schemes enjoy an improved achievable rate performance compared to the OFDM counterpart{\footnote{It should be noted that this conclusions does not contradict to the ones from~\cite{rezazadehreyhani2018analysis}, because the unitary transformation between different domains may not hold in the multiple access transmission, because each user only occupies limited resources~\cite{Ruoxi2022achievable}.}}.


\subsection{Integrated Sensing and Communications}
ISAC transmission has been widely recognized as an efficient approach to deal with the foreseeable coexistence between communication and radar~\cite{liu2020joint,liu2018mu}.
A key motivation for ISAC transmission designs is that both radar sensing and communication naturally have similar channel characteristics which can be exploited.
For example, let us consider a common downlink scenario in a mobile network, where the antennas for radar sensing and communication are co-located at the BS.
It is not hard to notice that the physical channel between the BS and user equipments (UEs) is the same for both radar sensing and communication, despite the fact that radar sensing is operated based on the received echoes at the BS after the \emph{round-trip} signal propagation, while signal detection for communication is based on the \emph{one-way} transmission from the BS to UEs.
It is worthwhile to notice that radar sensing carries out parameter estimations based on
the delay, Doppler, and angular features associated to resolvable paths, whose core idea aligns perfectly with the OTFS modulation for communication purpose.
The DD domain symbol multiplexing enables the direct interactions between the information symbols and the DD domain channel, whose channel response can be potentially inferred from the radar estimates in practice~\cite{yuan2021integrated}.
The synergistic ecosystem established by needs of communication and radar sensing has motivated us to consider the ISAC transmission design based on OTFS modulation.
Various lines of research works have been conducted in the literature. For example, the effectiveness of OTFS modulation for ISAC transmission has been evaluated in~\cite{Gaudio2020on}, where the authors have shown that the estimation error lower bounds for radar sensing can be achieved by using OTFS signals while maintaining a satisfactory communication performance. This work has then been extended to the case of MIMO transmissions~\cite{gaudio2020hybrid}, where a hybrid digital-analog beamformer is devised for both radar sensing and communication. In addition, the author in~\cite{gaudio2020hybrid} have also developed an efficient maximum-likelihood (ML) algorithm to facilitate target detection and parameter estimation.
In addition, a novel OTFS-based matched-filter algorithm for target range and velocity estimation for radar sensing has been proposed in~\cite{raviteja2019orthogonal}. Specifically, the proposed matched-filter algorithm takes advantages of the structures of DD domain effective channel matrix and has shown better estimation performance compared to the OFDM counterpart.
Furthermore, an ISAC-assisted OTFS system has been proposed in~\cite{yuan2021integrated}, where both uplink and downlink communications are considered. In particular, the authors proposed a novel DD domain channel estimation algorithm and introduced a message-passing based detection algorithm for uplink transmission. On the other hand, the downlink communication transmission is designed based on the channel state information (CSI) obtained from radar sensing, such that it can bypass the need of channel estimation and equalization at the receiver side.

The application of OTFS modulation in ISAC transmissions will be discussed in details in Chapter~8 of this thesis.









==> 9-MIMO_OTFS/MIMO_OTFS.tex <==
\chapter{Downlink Multiuser MIMO-OTFS Transmission using Tomlinson-Harashhima Precoding}\label{c:literature}

The literature review. This is a citation .



==> dissertation-sheet.tex <==
% this file is used by HDR these to generate the formal
% Thesis/Dissertation Sheet

\ThesisFamilyName{Li}
\ThesisGivenName{Shuangyang}
\ThesisOtherNames{} %if any, set to {} if not used

\ThesisAbbreviatedDegree{PhD}


\begin{ThesisAbstract}

\end{ThesisAbstract}

